Collaborating Foundation Models for Domain Generalized Semantic Segmentation

Domain Generalized Semantic Segmentation (DGSS) deals with training a model on a labeled source domain with the aim of generalizing to unseen domains during inference. Existing DGSS methods typically effectuate robust features by means of Domain Randomization (DR). Such an approach is often limited as it can only account for style diversification and not content. In this work, we take an orthogonal approach to DGSS and propose to use an assembly of CoLlaborative FOUndation models for Domain Generalized Semantic Segmentation (CLOUDS). In detail, CLOUDS is a framework that integrates FMs of various kinds: (i) CLIP backbone for its robust feature representation, (ii) generative models to diversify the content, thereby covering various modes of the possible target distribution, and (iii) Segment Anything Model (SAM) for iteratively refining the predictions of the segmentation model. Extensive experiments show that our CLOUDS excels in adapting from synthetic to real DGSS benchmarks and under varying weather conditions, notably outperforming prior methods by 5.6% and 6.7% on averaged miou, respectively. The code is available at : https://github.com/yasserben/CLOUDS

==> figs/plot_dataset_size.tex <==
\begin{tikzpicture}
\definecolor{darkslategray38}{RGB}{38,38,38}
\definecolor{lightgray204}{RGB}{204,204,204}
\begin{axis}[
    xlabel={Dataset Size (Number of Images)},
    tick align=outside,
    xtick pos=left,
    x grid style={lightgray204},
    xlabel=\textcolor{darkslategray38}{Number of images \(\displaystyle \longrightarrow\)},
    xmajorticks=true,
    xmin=50, xmax=25000,
    xmode=log,
    xtick style={color=darkslategray38},
    xtick={100,1000,10000},
    xticklabels={
      \(\displaystyle {100}\),
      \(\displaystyle {10^{3}}\),
      \(\displaystyle {10^{4}}\),
    },
    ytick={58, 59, 60, 61, 62},
    y grid style={lightgray204},
    ylabel=\textcolor{darkslategray38}{mIoU (in \%) \(\displaystyle \longrightarrow\)},
    ymajorgrids,
    ytick pos=left,
    ymajorticks=true,
    ytick style={color=darkslategray38},
    legend pos=north west,
    grid style=dashed,
    height=0.8\linewidth,
    width=\linewidth,
]

\addplot[
    color=blue,
    mark=square,
    ]
    coordinates {
    (100,58.2)(500,60.2)(1000,61.0)(5000,61.5)(10000,61.6)(20000,61.6)
    };
\legend{mIoU}
\end{axis}
\end{tikzpicture}

==> sec/Tables/ablation_sam.tex <==
\begin{table}[t]
\footnotesize
\centering
\setlength{\tabcolsep}{5.3pt}
\begin{tabular}{cccc|ccc}
\toprule
&\multicolumn{3}{c}{\textbf{Points}}& \multicolumn{3}{c}{\textbf{Threshold}}\\
% &\multicolumn{3}{c}{\textbf{Num_points} }& \multicolumn{3}{c}{\textbf{Threshold}}\\
&\textbf{5}  & \textbf{10} & \textbf{50} &  \textbf{0} & \textbf{5000} & \textbf{10000} \\ 
\midrule
\multicolumn{1}{c}{\textbf{mIoU}}& \textbf{61.5} & 60.9 &  60.0 &  44.5 & 61.5 & 61.3 \\ 
\bottomrule
\end{tabular}
\caption{Segmentation performance\steph{can we have a plot?}}
\label{table:ablation_sam}
\end{table}
